Accurate Uncertainty Estimation and Decomposition in Ensemble Learning

Ensemble learning is a standard approach to building machine learning systems that capture complex phenomena in real-world data. An important aspect of these systems is the complete and valid quantification of model uncertainty. We introduce a Bayesian nonparametric ensemble (BNE) approach that augments an existing ensemble model to account for different sources of model uncertainty. BNE augments a model's prediction and distribution functions using Bayesian nonparametric machinery. It has a theoretical guarantee in that it robustly estimates the uncertainty patterns in the data distribution, and can decompose its overall predictive uncertainty into distinct components that are due to different sources of noise and error. We show that our method achieves accurate uncertainty estimates under complex observational noise, and illustrate its real-world utility in terms of uncertainty decomposition and model bias detection for an ensemble in predict air pollution exposures in Eastern Massachusetts, USA.

==> preamble/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{wrapfig}

% Use fancyhdr package
\RequirePackage{multicol}
\RequirePackage{fancyhdr}
\RequirePackage{color}
%\RequirePackage{algorithm}
%\RequirePackage{algorithmic}
\RequirePackage{eso-pic} % used by \AddToShipoutPicture 
\RequirePackage{forloop}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage[numbers]{natbib}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}

\usepackage{lipsum}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2019} with \usepackage[nohyperref]{icml2019} above.
%\usepackage{hyperref}
\usepackage{comment}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% import external document
\usepackage{xr}

% custom macros
\usepackage{xcolor}

% theorem
\usepackage{amsthm}

\usepackage{"./macro/GrandMacros"}
\usepackage{"./macro/Macro_BIO235"}


==> sections/backup_experiments_metric.tex <==
\section{Experiments}
\label{sec:exp}


\subsubsection{Operating Characteristics}

To assess model's operating characteristics in prediction and uncertainty quantification, we consider both empirical measures that can be computed  in finite data, and also theoretical measures with respect to the ground truth distribution. We measure model's predictive performance using RMSE, both respect to the empirical observations in the testing dataset, and with respect to the theoretical mean in the ground truth distribution. To measure model's performance in uncertainty quantification, we consider the  empirical coverage probability, i.e. the observed probability $\hat{p}$ that the model's $p\%$ credible intervals cover the observations. If a model's uncertainty quantification is accurate, then the observed coverage probability $\hat{p}$ should be close to the claimed nominal coverage $p$, otherwise over-/under-estimated $\hat{p}$ indcates over-/under-confidence in model prediction. This gives rise \gls{CI} that assesses model's performance uncertainty quantification in the data by computing the difference between $\hat{p}$ and $p$ for a range of $p \in [0, 1]$:
\begin{align}
CI = \sum_{p \in [0, 1]}|\hat{p} - p|,
\label{eq:coverage_index}
\end{align}
Finally, we assess model's peformance in uncertainty quantification with respect to the ground-truth distribution by computing the $L_1$ distance:
\begin{align*}
L_1(F, \Fbb) = \sum_{\bx \in \Xsc} \int |F(y|\bx) - \Fbb(y|\bx)| dy
\end{align*}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\columnwidth]{example-image}
    \includegraphics[width=0.49\columnwidth]{example-image}
    \caption{Model's convergence behavior in prediction. \textbf{Left}: RMSE in testing data. \textbf{Right}: RMSE with respect to theoretical mean in ground truth distribution.}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.49\columnwidth]{example-image}
    \includegraphics[width=0.49\columnwidth]{example-image}
    \caption{Model's convergence behavior in uncertainty quantification. \textbf{Left}: Coverage Index in testing data. \textbf{Right}: $L_1$ with respect to ground truth distribution.}
\end{figure}


==> sections/backup_intro.tex <==
\section{Introduction}

Ensemble learning has a long history in areas such as robust engineering system design \citep{beyer_robust_2007} , financial investment management \citep{guiso_investment_1999}, and weather and climate forecast \citep{qian_uncertainty_2016}, where high-risk decisions and critical projections are made in the presence of noise and uncertainty. 
\begin{comment}
Given a set of expert-built base predictors $\{f_k\}_{k=1}^K$, ensemble methods output a predictor that commonly takes the form:
\begin{align}
y &= \sum_{k=1}^K f_k(\bx)\mu_k + \epsilon,
\label{eq:model_orig}
\end{align}
where $\bmu=\{\mu_k\}_{k=1}^K$ estimates the model's \textit{systematic component} describing the deterministic trend in the observations, and $\epsilon$ is the model's \textit{random component} describing the natural stochasticity surrounding the deterministic trend. Denoting $\Theta=\{\bmu, \epsilon\}$, the ensemble model 
%combines its systematic and random components to 
outputs a predictive distribution using its \gls{CDF} $F(y|\bx, \Theta)$.
\end{comment}
%In many applications, it is critical for the ensemble model to properly quantify the predictive uncertainty using the predictive distribution.
Failure in quantifying predictive uncertainty in these ensemble systems can lead to severe consequences \citep{amodei_concrete_2016}.
For example, a trading system predicting stock prices that fails to  capture the stochastic pattern in the stock price or is over-confident in its prediction can both lead to incorrect risk assessment for $P(y_{stock}< threshold)$, resulting in misinformed investment decisions.

% and an exposure assessment system for air pollution need to properly quantify both the fluctuation in pollution levels at a given location, and the model's changing confidence in prediction when switching between data-rich and data-sparse locations (e.g. regions with different number of air pollution monitors). 


% Consequently, the ensemble's predictive distribution $F(y|\bx)$ needs to incorporate both the natural, objectively existing stochasticity in the data, and its internal, subjective confidence in the ``correctness" of its prediction given current data and model specification at hand. In the language of \gls{UQ}, the model's description of the objective stochasiticity is known as the \textit{aleatoric uncertainty} and should be estimated to be consistent with data's empirical distribution, while the model's subjective uncertainty is known as the \textit{epistemic uncertainty} that arises due to the lack of data and knowledge about the data generation mechanism. For machine learning models, the epistemic uncertainty usually arise from two sources: the \textit{parametric uncertainty} in estimating parameters in the current model, and the \textit{structural uncertainty} in whether the current model specification is sufficient in describing the data distribution \citep{sullivan_introduction_2015} (See also Figure \ref{fig:unc_decomp}). For proper uncertainty quantification, an ensemble model's ability to distinguish and properly model all these three types of uncertainties is important.

%Consequently, %
To properly quantify predictive uncertainty, 
it is important for an ensemble learning system to recognize 
%and properly capture 
different types of uncertainties that arise in the modeling process. In machine learning modeling, two distinct types of uncertainties exist: \textit{aleatoric uncertainty} and \textit{epistemic uncertainty} \citep{kiureghian_aleatory_2009} (See Figure \ref{fig:unc_decomp}). Aleatoric uncertainty arises due to the stochastic pattern that objectively exists in the data, and is described by the model \gls{CDF} $F(y|\bx, \Theta)$. 
%It cannot be reduced even with infinite amount of data.
On the other hand, epistemic uncertainty arises due to our lack of knowledge about the data generation mechanism. 
A model's epistemic uncertainty can be reduced by collecting more data,  while aleatoric uncertainty is irreducible since it is inherent to the observation.
%concerns the uncertainty about the model at hand. 
%can be reduced by collecting more data. 
A machine learning model's epistemic uncertainty can arise from two sources \citep{sullivan_introduction_2015}: \textit{parametric uncertainty} that reflects uncertainty associated with estimating the  model parameters under the current model specification, which can be described by a Bayesian model's posterior $p(\Theta|y, \bx)$; and \textit{structural uncertainty} that reflects the uncertainty in whether the current model specification is sufficient in describing the data, i.e. whether there exists systematic discrepancy between model \gls{CDF} $F(y|\bx, \Theta)$ and data's empirical distribution $\bbF(y|\bx)$. 
%Both the parametric and structural uncertainties are \textit{epistemic uncertainty}, i.e. the uncertainty that arise due to lack of knowledge about the data generation mechanism, and can be reduced by collecting more data. On the other hand, aleatoric uncertainty cannot be reduced since it is inherent to the observation. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.6\columnwidth]{"./plots/uncertainty/tree"}
\caption{A decomposition of different types of uncertainty by the Bayesian Nonparametric Ensemble (BNE).}
\label{fig:unc_decomp}
\end{figure}

To this end, the goal of uncertainty estimation is to properly characterize both model's aleatoric and epistemic uncertainties. In regions in the feature space $\bx \in \Xsc$ which are well represented by the training data, the model's aleatoric uncertainty should acurately capture the data's empirical distribution (i.e. calibration \citep{gneiting_probabilistic_2007}), while in regions unexplored by the training data, the model's epistemic uncertainty should rise to reflect the model's lack of confidence in prediction (i.e. out-of-distribution generalization \citep{lakshminarayanan_simple_2016}). Furthermore, the structural uncertainty needs to be disentangled from the overall epistemic uncertainty. Since it is need to identify the sources of structural biases in the ensemble model, and to quantify how these biases impacts the the model output, which is necessary for the the continuous \textit{model validation} of an running ensemble system \citep{sargent_verification_2010, the_federal_reserve_board_of_governors_in_washington_dc._federal_2011}.

A comprehensive framework to accommodate
%treatment for
all three types of uncertainties is currently lacking in the ensemble learning  literature. We refer readers to Supplementary Section \ref{sec:related} for a full review and how our work is related to existing literature. Briefly, most existing methods handle the the aleatoric uncertainty using an assumed distribution family (e.g. Gaussian) \citep{lakshminarayanan_simple_2016, vandal_quantifying_2018}, not able to flexibly capture the wide range of stochastic patterns (e.g. asymmetry, heavy-tailedness, multimodal, or their combinations) in the real-world data. Also, few work exists in quantifying the epistemic uncertainty, especially the structural uncertainty (e.g. uncertainty stemming from the systematic bias among the base models contributing to the ensemble) in an ensemble model itself, although ensemble methods are often used to estimate epistemic uncertainty or mitigate structural uncertainty in the base models \citep{breiman_bagging_1996, lakshminarayanan_simple_2016, breiman_stacked_1996, pinder_efficient_2009}.

%For this purpose, the ensemble model's ability in distinguishing and properly capturing all three types of uncertainties is important. However, the existing ensemble methods usually quantify the aleatoric uncertainty using an assumed distribution family (e.g. Gaussian) \citep{lakshminarayanan_simple_2016, vandal_quantifying_2018}, falling short in flexibly capturing the wide range of stochastic patterns (e.g. asymmetry, heavy-tailedness, multimodal, or their combinations thereof) in the real-world data. On the other hand, while ensemble methods are often used to estimate epistemic uncertainty in its base models\citep{breiman_bagging_1996, lakshminarayanan_simple_2016, breiman_stacked_1996, pinder_efficient_2009}, there exists less work in quantifying the epistemic uncertainty in an ensemble model itself, especially in characterizing the structural uncertainty (e.g. uncertainty stemming from the systematic bias among the base models). We refer readers to Section \ref{sec:related} for a review.

%To this end, existing ensemble learning models are lacking in recognizing and properly quantifying different sources of model uncertainties. While there exists extensive work in addressing ensemble model's parametric uncertainty using Bayesian \citep{chipman_bayesian_1998, kim_bayesian_2012, mentch_quantifying_2014} and Monte Carlo methods \citep{tebaldi_claudia_use_2007, garaud_uncertainty_2012, sanderson_uncertainty_2018}, an ensemble model's aleatoric uncertainty is commonly modelled with an assumed distribution family  \citep{lakshminarayanan_simple_2016, vandal_quantifying_2018} (e.g. Gaussian), and therefore cannot flexibly incorporate the complex stochastic patterns (e.g. asymmetry, heavy-tailedness, multimodal) that  arise in the real-world data. One exception to this approach is the quantile random forest \citep{meinshausen_quantile_2006, taillardat_calibrated_2016} which robustly estimates the residual distribution using quantile regression, but is only developed for tree-based models \footnote{In Experiment section (Section \ref{sec:exp}), we develop a quantile-based ensemble for arbitrary base models $f_k$ and compare its performance with our approach}. Finally, while ensemble learning is commonly used as a method to mitigate structural uncertainty among the base models \citep{pinder_efficient_2009, parham_multimodel_2013, tyralla_incorporating_2016}, limited work exists in quantifying the structural uncertainty in the ensemble model itself \citep{parker_ensemble_2013} (e.g. uncertainty stemming from the systematic bias among the base models%, or the misspecification in the random component).

In this work, we aim to enable ensemble models to recognize and properly capture all three sources of predictive uncertainties, especially in the situation of realistic, complex (e.g. asymmetry, heavy-tailedness, multimodal, etc) observational noise. Our goals are (i) \textbf{Accurate Uncertainty Estimation} to properly characterize a model's aleatoric and epistemic uncertainties for the purpose of reliable prediction, and (ii) \textbf{Uncertainty Decomposition / Model Error Detection} to identify the sources of model bias and uncertainty in the current system, for the purpose of uncertainty reduction and model improvement. We consider the setting of continous-valued observations. 
%Specifically, we propose a principled augmentation framework for ensemble learning that flexibly quantifies an ensemble model's aleatoric, parametric and structural uncertainties using Bayesian nonparametric machinery, coupled with a decision-theoretic inference procedure that achieves accurate uncertainty estimation by caibrating model's estimate of aleatoric uncertainty (i.e. model \gls{CDF}) toward the empirical distribution of the data.  
Our contributions are:
%adopts an explicit decomposition of all three types of model uncertainties, offers flexible and accurate quantification of aleatoric uncertainty, and provides principled quantification of model's structural misspecification in its impact on model prediction. Our contributions are:
\begin{itemize}
\item We propose \gls{BNE}, an augmentation framework that mitigates the misspecification in the original ensemble model and flexibly quantifies all three sources of predictive uncertainties (Section \ref{sec:model}).
%\item We develope a principled approach in assessing the impact of different sources of model misspecification on model's predictive distribution (Section \ref{sec:impact_misspec}). 
\item We introduce \textbf{Calibrated Inference}, a novel decision-theoretic Bayesian inference procedure that lead to accurate estimate of aleatoric uncertainty and principled quantification of epistemic uncertainty. We also derive its variational approximation to enable scalable, end-to-end posterior updates (Section \ref{sec:inference}).
% We also derive the corresponding \gls{ELBO} to enable scalable, end-to-end posterior update using stochastic variational inference. We further show that with reasonable choice of variational family, this approach lead to accurate uncertainty quantification (Section \ref{sec:inference}).
\item 
%We evalute the proposed method's finite-sample operating characteristics in prediction and uncertainty quantification against common ensemble methods 
We demonstrate through simulation experiments that the proposed method achieves accurate uncertainty estimation under complex observational noise, offers improvement in predictive accuracy relative to the original ensemble, and is characterized by attractive convergence properties (Section \ref{sec:exp}).
\item We illustrate the real-world utility of our method in uncertainty decomposition and model bias detection for an ensemble system for particle pollution prediction in the greater Boston, U.S.A. area (Section \ref{sec:app_airpol}). 
\end{itemize}


%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------
%------------------------------------------


\begin{comment}
Ensemble learning forms the cornerstone of many machine learning systems interacting with real-world data
%, with applications ranging from online machine translation \citep{shazeer_outrageously_2017} to numeric weather forcasting \citep{gneiting_weather_2005}
. Given a set of base predictors $\{f_k\}_{k=1}^K$, ensemble methods provide a simple and effective approach to obtain a predictor with improved accuracy by leveraging the power of different $f_k$'s. In regression setting, such predictor commonly takes the form:
\begin{align}
f(\bx) &= \sum_{k=1}^K f_k(\bx)\mu_k + \epsilon,
\label{eq:model_orig_0}
\end{align}
where $\sum_{k=1}^K f_k(\bx)\mu_k$ is the ensemble prediction that is the  \textit{systematic component} of the model, and $\epsilon$ is a random variable describing the distribution of the outcome that is the \textit{random component} of the model.

%In the lifecycle of a ensemble learning system, practitioners usually  
%start from
%collect data
%improvement
%.

% Ensemble methods form the cornerstone of many machine learning systems interacting with real-world data \citep{okun_ensembles_2011}. {\color{red} (Example: in Translation \citep{devlin_bert:_2018} Numeric Weather forcast \citep{gneiting_combining_2013})}

%When deploying a pre-trained machine learning system in describing the real-world data, it is often of practical interest to understand the system's performance by quantifying different types of error and uncertainty that arise in model prediction, so we can rigorously assess the system's \textit{sufficiency} and \textit{reliability} in describing the real-world data, and at the same time pinpoint the the sources of modeling error that is most attributable to the model's lack of performance. 

%However, not all sources of uncertainty that arise in a machine learning application, only a subset is informative for .



%\citep{sullivan_introduction_2015}

%Furthermore, for the uncertainty decomposition to be meaningful.

%Two problems
%\begin{enumerate}
%\item 
%\item 
%\end{enumerate}

%In this work, we study in the context of ensemble learning. Ensemble learning  and have seen 

%form the cornerstone of many real-world machine learning systems ranging from large-scale machine translation \citep{shazeer_outrageously_2017} to numeric weather forcast \citep{gneiting_weather_2005}. 

%In this work we present a novel modeling framework to account for different sources of model uncertainty that arise in ensemble learning (see Figure \ref{fig:uncertainty}). Importantly, our method is capable of identify the ensemble model's structural uncertainty due to different types of model misspecification (e.g. misspecification in systematic component and in the random component), and precisely quantify the impact of different types of  model mispecification on the ensemble's predictive distribution.
\end{comment}

==> sections/backup_model.tex <==
\section{Bayesian Nonparametric Ensemble}
\label{sec:model}

In this section, we introduce the Bayesian Nonparametric Ensemble (BNE), a Bayesian nonparametric augmentation of the traditional ensemble model. It mitigates the original ensemble's misspecification in the systematic and the random components, offers an comprehensive account of different sources model uncertainty (Section \ref{sec:unc_decomp}), detects different types of model misspecification and quantifies how they impact  the model's predictive distribution (Section \ref{sec:impact_unc}).

Summarized in Figure \ref{fig:model}, \gls{BNE} augments the classic ensemble model in a manner similar to how \gls{GLM} augments classic linear regression. Specifically, given an observation pair $\{\bx, y\} \in \Xsc \times \Ysc$ and a set of base models $\Fsc = \{f_k\}_{k=1}^K$, a classic ensemble model assumes the form
\begin{align}
y &= \sum_{k=1}^K f_k(\bx)\mu_k + \epsilon,
\label{eq:model_orig}
\end{align}
where $\bmu=\{\mu_k\}_{k=1}^K$ are the ensemble weights assigned to each base model, and $\epsilon$ is a random variable describing the distribution of the outcome.
%where $\bmu=\{\mu_k\}_{k=1}^K$ are the ensemble weights estimating the model's \textit{systematic component} describing the deterministic trend in the observations, and $\epsilon$ is the random variable describing model's \textit{random component} describing the natural stochasticity surrounding the deterministic trend.
BNE generalizes this classic ensemble model by first augmenting its \textit{systematic component} by adding to it a nonparametric residual process $\delta(\bx)$ to mitigate the systematic prediction bias among the base models. Denoting $\Phi=\{ \bmu, \epsilon, \delta \}$, this systematic component model outputs a \gls{CDF} $F_S(y|\bx, \Phi)$. \gls{BNE} then augments the model's \textit{random component} (i.e. the model CDF) by mapping  $F_S$ to the empirical CDF $\Fbb$ with a nonparametric "link" function $G$ such that $\Fbb = G \circ F_S$. 
%Consequently,
To summarize, the full model for \gls{BNE} takes below form:
%the form in Figure \ref{fig:model}, 
\begin{figure}[ht]
\begin{alignat*}{4}
\mbox{Random Component}& \;\;
&& \;\; y | \bx && \sim \; &&  \Fbb(y|\bx)
\\
\mbox{Link Function}& \;\;
&& \Fbb(y|\bx) &&=  && G \circ F_S(y|\bx, \Phi)
\\
\mbox{Systematic Component} & \;\;
&& \quad y &&= \; && 
\sum_{k=1}^K f_k(\bx) \bmu_k
+ \delta(\bx) 
+ \epsilon,
%\label{eq:model}
\end{alignat*}
\caption{Bayesian Nonparametric Ensemble}
\label{fig:model}
\end{figure}

The overall model \gls{CDF} is $F(y|\bx, \Phi, G) =  G \circ F_S(y|\bx, \Phi)$, where $\circ$ denotes function evaluation. Further, the expression for model's \gls{PDF} is:
\begin{align}
f(y|\bx,G, \Phi) = g(F_S(y|\bx, \Phi)) * f_S(y|\bx, \Phi)
\label{eq:likelihood}
\end{align}
where $g$ is the derivative of $G$ with respect to $F_S$.

\subsection{Prior specification} 
\gls{BNE} contains four model parameters: the $\bmu=\{\bmu_k\}_{k=1}^K$ (ensemble weights) and $\bepsilon$ (observation noise) from the original ensemble, and $G$ (link function) and $\bdelta$ (residual process) that  augments the original model by addressing its misspecifications. In general, we leave $\bmu$ and $\bepsilon$ to follow the same specification as in the original ensemble model (\ref{eq:model_orig}). For the simplicity of exposition, in the rest of this section we assume $\bmu$ and $\bepsilon$ follow independent Gaussian priors, which corresponds to a classic stacked generalization model for Gaussian outcome \citep{breiman_stacked_1996}. However our framework can be readily adapted to other specifications for $\bmu$ and $\bepsilon$.

We place Bayesian nonparametric priors on $\bdelta$ and $G$ so they flexibly mitigate the model misspecification in the 
%systematic and random component of the 
original ensemble (\ref{eq:model_orig}), and at the same time account for the model's structural uncertainty. Importantly, we want to specify $\bdelta$ and $G$ in such a way that, in regions well represented by the training data, $\bdelta$ flexibly mitigates the systematic bias in the base models while $G$ calibrates the model \gls{CDF} to the empirical distribution. However, in regions outside training data (i.e. the out-of-distribution regions \citep{lakshminarayanan_simple_2016}), $\bdelta$ and $G$ should leave the predictions of the original ensemble (\ref{eq:model_orig}) intact so it does not harm the out-of-distribution behavior of the original model, but at the same time, posterior uncertainties in $\bdelta$ and $G$ should elevate naturally to reflect model's increasing epistemic uncertainty. 

For this purpose, we place on $\delta$ the Gaussian process prior with zero mean function $\bzero(x)=0$, and recommend using shift-invariant kernels as the kernel function. Shift-invariant kernels are well suited for quantifying epistemic uncertainty, since their predictive variance is explicitly characterized by the distance from the training data, therefore their predictive uncertainty rise naturally at locations far from training data \citep{rasmussen_gaussian_2006}. 

We place on $G$ also the Gaussian process prior, but with non-negativity constraint on $G$'s derivative $g$ so the final model \gls{CDF} $F=G \circ F_S$ is strictly monotonic (see Appendix \ref{sec:mono_gp} for detail)\citep{riihimaki_gaussian_2010}. Failure to account for the  monotonicity in $G$ leads to negative estimate in model \gls{PDF} (\ref{eq:likelihood}), rendering the classic log-likelihood based inference impossible. We use identity function $I(x)=x$ as the  mean function for $G$, so it does not interfere with the out-of-distribution behavior of original ensemble. That is, in regions outside training data, $G$ will fall back to identity function such that $F = G \circ F_S = F_S$. We recommend using Gaussian \gls{RBF} as the kernel function for $G$ due to both its univeral approximation property (i.e. able to approximate arbitrary continous \glspl{CDF} over the compact support)\citep{micchelli_universal_2006} and its ability in quantifying epistemic uncertainty (since it belongs to the shift-invariant kernel family). To summarize:
\begin{alignat*}{2}
G &\sim mono GP(I, k_G); \quad 
 &&\bdelta  \sim GP(\bzero, k_\delta); \\
\{\bmu_k\}_{k=1}^K &\stackrel{indep}{\sim} N(0, \sigma_k); \quad
&&\epsilon \sim N(0, \sigma_{\bepsilon}^2),
\end{alignat*}
A summary of the full model is shown in Figure \ref{fig:plate}.  For notational convenience, in the rest of the paper we will denote the collection of BNE's model parameters as $\Theta=\{\Phi, G\}$, where recall $\Phi=\{\mu, \epsilon, \delta\}$ are parameters for \gls{BNE}'s systematic component.

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\columnwidth]{"./plots/model/plate/plate"}
\caption{Plate Diagram for BNE}
\label{fig:plate}
\end{figure}

Compared to a classic Gaussian process model who is nonparametric in the systematic component but parametric in the random component (i.e. Gaussian) \citep{rasmussen_gaussian_2006}, BNE is \textit{fully nonparametric} since it does not assume its random component to follow any parametrized distribution family, but instead models it nonparametrically using $G$. 

%Consequently, it improves the model's capacity in both prediction and in uncertainty quantification by unbiasedly estimating the empirical distribution $\Fbb$.

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.155\textwidth}
        \includegraphics[width=\textwidth]{"./plots/model/ensemble_density_fit"}
    \end{subfigure}
    \begin{subfigure}{0.155\textwidth}
        \includegraphics[width=\textwidth]{"./plots/model/ensemble_posterior_mean"}
    \end{subfigure}    
    \begin{subfigure}{0.155\textwidth}
        \includegraphics[width=\textwidth]{"./plots/model/ensemble_posterior_sample"}
    \end{subfigure}    
    \caption{Toy example illustrating impact of $G$ on model's posterior predictive distribution. 
     \textbf{Dashed Line}: True Density $P(y|\bx)$, \textbf{Black Ticks}: Observations,
     \textbf{Red Shade}: Posterior distribution of $\sum_k f_k \mu_k$, \textbf{Grey Shade}: $F_S(y|\bx)$, \textbf{Blue Shade}: Posterior mean of $G \circ F(y|\bx)$}
    \label{fig:unc_0d}
\end{figure}


To further illustrate the role $G$ play in the BNE's ability in accurately characterizing an outcome distribution, we consider a toy example where we run  \gls{BNE} model both with and without $G$ to predict $y$ at a fixed location of $\bx$ (i.e. estimating the conditional distribution $\Fbb(y|\bx)$ at fixed location of $\bx$) where $y|\bx \sim Gamma(1.5, 2)$ (Figure \ref{fig:unc_0d}). Notice that the \gls{BNE} model without $G$ (i.e. the systematic-component model) is in fact still a very flexible model, since it follows a hierarhical Gaussian process with mean $\sum_{k=1}^K f_k(\bx)\mu_k$ and kernel function $k_\delta(\bx, \bx') + \sigma_\epsilon^2$. However, as shown in Figure \ref{fig:unc_0d}, the posterior distribution of the systematic-component model (grey shade) failed to capture the skewness in data's empirical distribution, and consequently yields a biased \gls{MAP} estimate due to its restrictive distributional assumptions. On the other hand, the full BNE model is able to calibrate its predictive distribution (blue shade) toward the empirical distribution of the data using $G$, and consequently produces better quantification of $\Fbb(y|\bx)$ and improved \gls{MAP} estimate.

\begin{comment}
\textbf{Posterior Likelihood} Recall the model \gls{CDF} is $F(y|\bx, G, \Phi)=G \circ F_S(y|\bx, \Phi)$, where $F_S(y|\bx, \Phi)$ is the model \gls{CDF} for the model's systematic component in Figure \ref{fig:model}. Therefore the expression for model \gls{PDF} is:
\begin{align}
f(y|\bx,G, \Phi) = g(F_S(y|\bx, \Phi)) * f_S(y|\bx, \Phi)
\label{eq:likelihood}
\end{align}
where $g$ is the derivative of $G$ with respect to $F_S$, and is explicitly modeled by the monotonic Gaussian process $f(G) = P(\Csc|g)P(g, G)$ (see (\ref{eq:mono_gp})). Consequently, one can perform posterior inference using any standard inference algorithm with respect to the full posterior:
\begin{align}
f(G, \Phi|y, \bx) \propto f(y|\bx, G, \Phi)f(G)f(\Phi).
\label{eq:posterior}
\end{align}
We discuss the inference for \gls{BNE} in depth in Section \ref{sec:inference}.
\end{comment}

==> sections/backup_model_uq.tex <==
\section{Uncertainty Quantification with \gls{BNE}}
\label{sec:uq}

Using \gls{BNE}, we are able to achieve the two canonical goals of \gls{UQ} \citep{u.s._department_of_energy_scientific_2009}: (1) \textbf{Uncertainty Decomposition} to distinguish the contribution of different sources of model uncertainties in driving the overall predictive uncertainty, and (2) \textbf{Model Bias Detection} to identify different types of model bias in the current ensemble model, and quantify how they impact  the model's predictive distribution.

\subsection{Uncertainty Decomposition}
\label{sec:unc_decomp}

% We now consider the role that each of \gls{BNE}'s model parameters play in accounting for different types of model uncertainties, and show how to precisely quantify the magnitude of these uncertainties by decomposing the posterior uncertainty of \gls{BNE}'s predictive distribution. 
As shown in Figure \ref{fig:unc_decomp}, the posterior uncertainty in each of the four model parameters $\{\bmu, \bdelta, G, \bepsilon\}$ accounts for a important source of model uncertainty: the posterior uncertainty in $\bmu$ accounts for the \textit{parametric uncertainty},
%, i.e. the model's uncertainty about what are the exact values that the ensemble parameters should take
the uncertainties in $\bdelta$ and $G$ account for the \textit{structural uncertainties} in its prediction function and distribution function, 
%i.e. the uncertainty about whether the model structure in the systematic and random components are correctly specified to sufficiently describe the data-generation mechanism. Both of these two types of uncertainties are \textit{epistemic uncertainty} in that they arise due to our lack of data and knowledge about the data generation mechanism, and can be reduced by collecting more data. On the other hand, 
and the uncertainty in $\bepsilon$ accounts for the \textit{aleatoric uncertainty} 
%which reflects the natural stochasticity inherent in the observation (e.g. due to measurement error, and cannot be reduced even with infinite amount of data\citep{sullivan_introduction_2015}
. 

Consequently, all three types of uncertainties are present in  \gls{BNE}'s predictive distribution, and can be rigorously quantified through a decomposition of the overall predictive variance, that is:
\begin{align}
VAR_y & (y |\bx)  = \nonumber \\
& \underbrace{
VAR_G \Big[ E_y(y|\bx, G) \Big]}_{structural, G} + 
\underbrace{ 
E_G\Big[ 
VAR_{\bdelta}  \big[ E_y( y| \bx, G,\delta) \big] \Big]
}_{structural, \bdelta} + 
\nonumber \\
& 
\underbrace{
E_{G, \bdelta} \Big[ VAR_{\bmu} \big[ E_y(y|\bx, G, \bdelta, \mu) \big] \Big]}_{parametric, \bmu}
 + 
\nonumber \\
& 
\underbrace{
E_{G, \bdelta, \mu} \Big[ VAR_y(y|\bx, G, \bdelta, \mu) \Big] 
}_{aleatoric, \bepsilon},
\label{eq:unc_decomp}
\end{align}
where for $\Omega \subset \{\bmu, \bdelta, G, \bepsilon\}$ a subgroup of model parameters, $E_{\Omega}$ and $VAR_\Omega$ denotes the expectation and variance with respect to $\Omega$'s posterior distribution
%, and $\bar{G} = E_G(G)$ denotes the posterior mean of $G$ 
(see Supplementary \ref{sec:unc_decomp_deriv} for derivation). In particular, %we see that 
%the expression for the aleatoric uncertainty in (\ref{eq:unc_decomp}) indeed quantifies only the contribution of $\epsilon$ to the overall uncertainty, as this expression describes model's average posterior belief (i.e. the posterior mean) in the conditional variance of $y|\bx$ holding all the other non-$\bepsilon$ parameters fixed. Furthermore, 
although the specification for $\epsilon$ can be restrictive in its prior distribution, this expression shows us that the model's quantification of the aleatoric uncertainty via $\epsilon$ is in fact flexible in the posterior distribution
%and is able to quantify heterogeneous and complex noise 
due to its dependency on the nonparametric link function $G$. 
%All expressions in (\ref{eq:unc_decomp}) can be computed  efficiently through Monte Carlo integration given posterior sample (see  Supplementary \ref{sec:unc_decomp_est}). 
We illustrate examples of such decomposition in the experiments (Section \ref{sec:exp_decomp}).

\subsection{Uncertainty-aware Detection of Model Biases}
\label{sec:impact_unc}

%An important goal of uncertainty quantification is to quantify the impact of different sources of model error on the model output in order to help practitioner to identify the most effective strategy for model improvement. 
%For example, the uncertainty decomposition in (\ref{eq:unc_decomp}) shows the contribution of different types of uncertainties in predictive variance. Using this information, we can identify regions in $\bx \in \Xsc$ with the highest level of parametric uncertainty, so we can collect additional data in that region in order to reduce variance in the exisiting model in the most efficient manner possible. %Otherwise we may waste resource on regions with high overall uncertainty due only to high level of aleatoric uncertainty.
%To this end, using posterior estimates of $G$ and $\delta$, \gls{BNE} is able to explicitly characterize the impact of systematic-component and random-component misspecification on different statistical properties of the predictive distribution. Furthermore, it communicates its degree of posterior belief on the said characterization using the structural uncertainty. 

%Using posterior estimates of $G$ and $\delta$, \gls{BNE} is able to detect  different types of model biases in its predictive distribution 
%(e.g. biased predictive mean, under-estimated  predictive uncertainty, failing to incorporate multimodality, etc), 
%and quantify its posterior belief for the detected biases, 
%attributing such biases back to the misspecification in its prediction function, 
%thereby providing actionable information in facilitating effective model improvement. 

\textbf{Impact on Predictive Mean} 
To assess the impact of model biases on predictive mean, we can estimate:
\begin{alignat}{2} 
D_{\delta} \big( y | \bx \big) = 
E \big(y|\bx, \delta \big) - E \big( y|\bx, \delta=\bzero \big) \nonumber \\
D_{G} \big( y | \bx \big) =
E \big(y|\bx, G \big) - E \big( y|\bx, G=\bI \big)
\label{eq:impact_misspec}
\end{alignat}
where $\bzero$ and $\bI$ indicates the zero function $\bzero(x)=0$ and the identity function $\bI(x)=x$ as before. These two quantities above can be interpreted as capturing the difference in the posterior predictive mean, if we do not account for model bias in the prediction function (by fixing $\delta=\bzero$) or in the distribution specification (by fixing $G=\bI$). Further, since both $G$ and $\delta$ are random quantities that accounts for model's structural uncertainty, $D_{\delta}$ and $D_{G}$ are also random quantities for which their posterior distributions can be estimated. Consequently, we can assess the model's posterior belief in whether these differences are different from zero by estimating $P\Big( D_{\delta} \big( y | \bx \big) > 0 \Big)$ and $P\Big(D_{G} \big( y | \bx \big) > 0 \Big)$, i.e. the percentiles of $0$ in the posterior distribution of $D_{\delta}$ and $D_G$. Values close to 0 or 1 indicates strong evidence in that the model bias impacts the predictive mean, while values close to 0.5 indicates that the posterior distributions of $D_{\delta}$ / $D_G$ are roughly centered around zero. In practice, both expressions in (\ref{eq:impact_misspec}) can be expressed analytically in terms of $F_S$
%\begin{align*}
%D_{G} \big( y | \bx \big) &= \int \Big[ F_S(y|\bx) - G\circ F_S(y|\bx) \Big] dy
%\\
%D_{\delta} \big( y | \bx \big) &= 
%\delta(\bx) + D_{\bar{G}} \big( y | \bx \big) - D_{\bar{G}} \big( y | \bx, \delta=\bzero \big).
%\end{align*}
(see Supplementary \ref{sec:unc_impact_app} for detail).
%These quantities can be computed efficiently in practice through Monte Carlo integration (see Supplementary \ref{sec:unc_impact_app} for derivation).

\textbf{Impact on Predictive Distribution's Other Properties} 
We can generalize the above approach to describe the impact of model bias on a certain property of the predictive distribution (e.g. predictive variance, skewness, multi-modality, etc). Specifically, given a summary statistic $s(y)$ that describes certain property of the predictive distribution, we can assess the impact of misspecification on such property by estimating
\begin{alignat*}{2}
& D_{\delta} \big( s(y) | \bx \big) = 
 E \big(s(y)|\bx, \delta \big) - 
 E \big( s(y)|\bx, \delta=\bzero \big) 
 \nonumber\\
& D_{G} \big( s(y) | \bx \big) = 
E \big(s(y)|\bx, G \big) - 
E \big( s(y)|\bx, G = \bI \big),
%\label{eq:impact_misspec_general}
\end{alignat*}
and assess the degree of posterior belief for these differences using $P\Big( D_{\delta} \big( s(y) | \bx \big) > 0 \Big)$ and $P\Big( D_{G} \big( s(y) | \bx \big) > 0 \Big)$. 
%Similar to (\ref{eq:impact_misspec}), above expressions also adopt analytical form in terms of $F_S$
%(see Supplementary \ref{sec:unc_impact_app} for detail)
Example properties of data distribution that relevant in practice include:
\begin{itemize}
\item \textbf{Predictive Uncertainty}, which can be assessed using predictive variance with summary statistic $s(y) = (y-E(y))^2$.
\item \textbf{Asymmetry}, which can be assessed by skewness with summary statistic $s(y) = \Big(\frac{y-E(y)}{\sqrt{Var(y)}}\Big)^3$. 
Positive skewness indicates heavy tail in the positive direction (e.g. exponential or Gamma).
\item \textbf{Multi-modality}, which can be assessed by kurtosis with summary statistic $s(y) = \Big(\frac{y-E(y)}{\sqrt{Var(y)}}\Big)^4$ 
%or other test statistics that are designed to measure multimodality
\citep{bajgier_powers_1991, dagostino_tests_1973, yap_comparisons_2011}.
\end{itemize}

%Consequently, using the methods developed in this section, BNE is able to quantify posterior evidence for different types of lack of fit in model's predictive distribution (e.g. bias in predictive mean, under-estimation in predictive uncertainty, failing to incorporate the heavy-tail/multimodality in the data distribution, etc), and furthermore, attributing such lack of fit back to the misspecification in different model components, thereby providing actionable information in facilitating effective model improvement. 
%In Section \ref{sec:exp}, we apply above method to assess the consequence  of model bias 
%illustrate examples of such impact quantification in detecting model's lack of fit under complex observation noise. 
In Section \ref{sec:app_airpol}, we apply above method to detect the systematic bias shared among base models in a real-world ensemble system for air pollution prediction.

==> sections/bne_consistency.tex <==
\begin{proof}
Analogous to Theorem 3.2 of \cite{van_der_vaart_rates_2008}, we show Theorem \ref{thm:bne_consistency} by invoking Theorem 2.1 of \cite{ghosal_convergence_2000} which shows the posterior consistency for general Bayesian models, provided that  certain conditions on the model likelihood and the prior distribution are satisfied (i.e. condition (\ref{eq:conv_cond_orig_3})-(\ref{eq:conv_cond_orig_1}) in below theorem). For completeness, we state the theorem below:

\begin{theorem_app}[Posterior Consistency for General Bayesian Models]
Let $\{y_i, \bx_i\}_{i=1}^n \sim P^*(y|\bx)$, and let $P \sim \Pi_n$ be a sequence of prior probability with support on $B$, and $||.||$ a metric on $B$. Denote $N(\epsilon, B, d)$ the $\epsilon$-packing number for set $B$ with respect to metric $||.||$, also denote $KL(P, P^*)$ the \gls{KL} divergence, and $V(P, P^*)=E^*\big(log(\frac{P}{P^*})^2\big)$ the $L_2$ metric for log likelihood ratio between $P$ and $P^*$.

Suppose that for a sequence $\epsilon_n \rightarrow 0$ and $n \epsilon_n^2 \rightarrow \infty$, a constant $C$ and a sequence of set $B_n$, we have:
\begin{align}
    log \, N(\epsilon_n, B_n, ||.||) 
    &\leq n\epsilon_n^2 
    \tag{\ref{thm:post_conv}-I}
    \label{eq:conv_cond_orig_3} \\
    \Pi_n(B \backslash B_n) 
    &\leq exp(-n\epsilon^2_n(C+4))
    \tag{\ref{thm:post_conv}-II}
    \label{eq:conv_cond_orig_2} \\
    \Pi_n \Big( KL(P, P^*) \vee V(P, P^*) \leq \epsilon_n^2 \Big)
    &\geq exp(-n \epsilon_n^2 C)
    \tag{\ref{thm:post_conv}-III}
    \label{eq:conv_cond_orig_1} 
\end{align}
Then for sufficiently large $M$, we have that in probability:
\begin{align*}
    \Pi_n \Big( d(P, P_0) \geq M \epsilon_n \Big| \{y_i, \bx_i\}_{i=1}^n \Big) \rightarrow 0
\end{align*}
\label{thm:post_conv}
\end{theorem_app}
Therefore to show posterior consistency, only need to show the three conditions in above theorem hold. To this end, we make use of the below theorem from \cite{liu_gaussian_2019} which derives the aforementioned conditions for \gls{CGP}. We state this theorem below:
\begin{theorem_app}[Conditions for Posterior Consistency in \gls{CGP}]
Let $g$ be a Borel measurable, zero-mean constratined Gaussian random element in a separable Banach space $(\Bbb, ||.||_\infty)$ with \gls{RKHS} $(\Hsc_k, ||.||_{\Hsc_k})$. Define the concentration function $\psi_{g^*}(\epsilon) = \inf_{\hat{g} \in \Hsc_k, ||\hat{g} - g^*||_\infty \leq \epsilon} ||\hat{g}||^2_{\Hsc_k} - log \, P(||g||_\infty \leq \epsilon)$. 

For any number $\epsilon_n > 0$ satisfying $\psi_{g^*}(\epsilon_n) \leq n\epsilon_n^2$, and any constant $C \geq 1$ with $e^{-Cn\epsilon_n^2} < \frac{1}{2}*  \frac{E(f(\Csc|g))}{E(||g||_{\Hsc_k}^2)\vee 1}$, for $g^*$ a function contained in the closure of $\Hsc_k$ in $\Bbb$ that is $\epsilon_n$-feasible, there exists a measurable set $B_n \subset \Bbb$ such that:
\begin{align}
log \, N(2 \epsilon_n, B_n, ||.||) &\leq 2 C n \epsilon_n^2 
    \tag{\ref{thm:cgp_conv}-I}
\label{eq:conv_cond_3} \\
P(g \not\in B_n) &\leq e^{-Cn\epsilon_n^2} 
    \tag{\ref{thm:cgp_conv}-II}
\label{eq:conv_cond_2} \\
P(||g - g^*|| < 2\epsilon_n) &\geq e^{-n\epsilon_n^2} 
    \tag{\ref{thm:cgp_conv}-III}
\label{eq:conv_cond_1} 
\end{align}
\label{thm:cgp_conv}
\end{theorem_app}
%This is a result that is analogous to Theorem 2.1 in \cite{van_der_vaart_rates_2008} but designed for the constrained Gaussian process. Similar to \cite{van_der_vaart_rates_2008}, there exists a slight mismatch between  conditions (\ref{eq:conv_cond_3}) and (\ref{eq:conv_cond_orig_3}) in terms of an additional multiplicative constant $2C$, which, as commented by the original author, is of no substantive importance since we are only interested in rates of convergence.
Consequently, to show the posterior consistency for \gls{BNE} with respect to the $L_2$ metric $E^*\big(||F - F^*||_2\big)$, we only need to show the three conditions in Theorem \ref{thm:post_conv} is satisfied by making use of Theorem \ref{thm:cgp_conv}. 

Notice for sufficiently small $\epsilon_n$, $F^*$ is $\epsilon_n$-feasible (i.e. $E(f(\Csc|F^* + s)) > E(f(\Csc|s))$ where $s$ is a bounded random noise $s \sim GP(0, k)$ and $||s|| < \epsilon_n$, see \cite{liu_gaussian_2019} for full definition) since the zero function $\bzero(x)=0$ lies on the boundary of the constrain set $\Csc$, therefore we can apply Theorem \ref{thm:cgp_conv} for \gls{BNE}. Only left to check if the three conditions in Theorem \ref{thm:post_conv} are satisfied by making use of Theorem \ref{thm:cgp_conv}. It is easy to see that conditions \ref{eq:conv_cond_orig_3} and \ref{eq:conv_cond_orig_2} are satisfied by \ref{eq:conv_cond_3} and \ref{eq:conv_cond_2}. Therefore only need to show that condition \ref{eq:conv_cond_orig_1} also holds. To this end, notice that  by Lemma 3.2 of \cite{van_der_vaart_rates_2008} the $KL(P, P^*)$ and $V(P, P^*)$ metrics in condition (\ref{eq:conv_cond_orig_1}) is upper bounded by the $L_2$ metric (denoted as $||.||$) in equation (\ref{eq:conv_cond_1}) up to a multiplicative constant. Therefore \ref{eq:conv_cond_1} implies \ref{eq:conv_cond_orig_1}. As a result, the three conditions in Theorem \ref{thm:post_conv} are satisfied, which implies posterior convergence.
\end{proof}

==> sections/discussion.tex <==
\section{Discussion and Future Directions}
\begin{enumerate}
\item High-dimension
\item Correlated outcome.
\end{enumerate}

==> sections/experiments_metric.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\columnwidth]{"./plots/metric/metric_rmse"}
    \includegraphics[width=0.45\columnwidth]{"./plots/metric/metric_l1"}
    \caption{Model's convergence behavior in prediction and uncertainty quantification with respect to data-generating distribution. 
    \textbf{Left}: RMSE. 
    \textbf{Right}: $L1$ distance $L(F, F^*)=\sum_{\bx \in \Xsc} \int |F(y|\bx) - F^*(y|\bx)| dy$.
    }
    \label{fig:metrics}
\end{figure}

\paragraph{Operating Characteristics} 
%To assess model's operating characteristics in prediction and uncertainty quantification, we measure model's predictive performance using RMSE with respect to the mean in the ground truth distribution, and measure model's performance in uncertainty quantification using the $L_1$ distance between the model's predictive \gls{CDF} $F$ and the ground-truth distribution $F^*$: $L(F, F^*)=\sum_{\bx \in \Xsc} \int |F(y|\bx) - F^*(y|\bx)| dy $.
%, we consider the  empirical coverage probability, i.e. the observed probability $\hat{p}$ that the model's $p\%$ credible intervals cover the observations. If a model's uncertainty quantification is accurate, then the observed coverage probability $\hat{p}$ should be close to the claimed nominal coverage $p$, otherwise over-/under-estimated $\hat{p}$ indcates over-/under-confidence in model prediction. This gives rise \gls{CI} that assesses model's performance uncertainty quantification in the data by computing the difference between $\hat{p}$ and $p$ for a range of $p \in [0, 1]$:
%\begin{align}
%CI = \sum_{p \in [0, 1]}|\hat{p} - p|,
%\label{eq:coverage_index}
%\end{align}
%Finally, we assess model's peformance in uncertainty quantification with respect to the ground-truth distribution by computing the $L_1$ distance:
%\begin{align*}
%L_1(F, \Fbb) = \sum_{\bx \in \Xsc} \int |F(y|\bx) - \Fbb(y|\bx)| dy
%\end{align*}

We benchmark \gls{BNE} against its abalated version (\textbf{BAE}) as well as both classic and recent Bayesian ensemble methods: the classic \gls{BME} \citep{waterhouse_bayesian_1996} which adaptively combines the predictive distributions using softmax-transformed Gaussian weights as $\sum_k \pi_k(\bx)\phi(y|f_k, \sigma_k)$, and also the recent \gls{stack} \citep{yao_using_2018} which uses non-adaptive weights $\sum_k \pi_k\phi(y|f_k, \sigma_k)$ but calibrates $\pi_k$ using leave-one-out cross validation. We vary sample size between 100 and 1000, and and repeat the simulation 50 times for each sample setting. Figure \ref{fig:metrics} shows the average RMSE (Top) and $L_1$ distance (Bottom) across the different sample size settings. We first observe that the patterns of change in RMSE and $L_1$ distance with respect to sample size are very similar, this is expected since by the classic mathematical statistics result $E(y|\bx)=\int [I(y>0)-F(y|\bx)] dy$ \citep{muldowney_darth_2012}, model's prediction performance is directly associated with its quality in estimating $F(y|\bx)$. Consequently, the improvement in estimating $F$ is reflected directly in the improvement in RMSE. As expected, the predictive accuracy and $L_1$ distance of both \textbf{stack} and \textbf{BAE} stablized at higher values due to the lack of adaptivity to the heterogneity in the data, producing biased model estimates even in large sample. On the other hand, \gls{BME} and \gls{BNE} is able to continuously improve due to the adaptivity in their distribution assumptions. We also observe \gls{BNE} is shown to perform better in larger sample, due most likely to its flexibility in distribution assumption (purely parametric) when compared to that of the \gls{BME} (a $K$-mixture of Gaussians).


%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.49\columnwidth]{example-image}
%    \includegraphics[width=0.49\columnwidth]{example-image}
%    \caption{Model's convergence behavior in uncertainty quantification. \textbf{Left}: Coverage Index in testing data. \textbf{Right}: $L_1$ with respect to ground truth distribution.}
%\end{figure}


==> sections/inference.tex <==
\section{Posterior Inference}
\label{sec:inference}

\subsection{Posterior Likelihood}
To ensure efficient posterior sampling, we integrate out $G$ and $\delta$ from the model posterior, and express the model compactly as $F^*(y|\bx) = F(y|\bx, \mu)$ with prior:
\begin{align}
     \quad
    F | \mu \sim CGP\big( \Phi_\epsilon(y|\bx, \mu), k_G \big), \quad
    \mu | \omega \sim GP\big( \sum_k f_k(\bx) \omega_k, k_\mu \big),
\label{eq:compact_bne_model}
\end{align}
and to avoid parameter non-identifiability, we orthogonalize $k_G$ and $k_\mu$ with respect to their mean functions $\Phi_\epsilon$ and $\sum_k f_k(\bx)$ \citep{reich_effects_2006, maceachern_comment_2007}. Specifically, given a kernel matrix $\bK$ generated by the kernel function $k$, and a mean function matrix $\bF_{N \times K}$ that corresponds to the $K$ mean functions evaluated at $N$ data points, we can compute the orthogonal projection matrix to the residual space of mean function as $\bP_{N \times N} = \bI - \bF(\bF^\top\bF)^{-1}\bF^\top$ where $\bF_{N \times K}$, and compute the orthogonalized kernel matrix as $\bK = \bP\bK\bP^\top$ \citep{reich_effects_2006}.

Consequently, given observations $\Dsc=\{y_i, \bx_i\}_{i=1}^N$, denoting 
%$\Phi$ the standard Gaussian \gls{CDF} and 
$\phi(.|\bm, \bS)$ the Gaussian \gls{PDF} with mean $\bm$ and covariance function $\bS$, \gls{BNE}'s model posterior $p_{\Dsc}$ is a simple product of model \gls{PDF}s $f = \deriv{y} F$ and Gaussian distribution functions:
\begin{align}
    p_{\Dsc}(F, \mu) 
    &\propto 
    \Big[\prod_{i=1}^N f(y_i|\bx_i, \mu) \Big] * 
    p\big(f\big|\mu \big) * p\big(\mu\big|\omega \big) * p\big(\omega\big),
    \label{eq:bne_posterior}
    % \\
    % &\propto 
    % \Big[\prod_{i=1}^N f(y_i|\bx_i, \mu) \Big] * 
    % \Big[\phi \big( f \big| \phi(y_i|\bx_i, \mu), \bK_G \big)\Big] * 
    % \phi \Big( \mu | \sum_k f_k \omega_k, \bK_\mu \Big) * 
    % \phi \Big( \bomega | 0, \sigma^2_\omega \bI \Big)
\end{align}
where $p(\mu \big| \omega)$ is the standard \gls{GP} likelihood, and $p(\omega)$ is the zero-mean Gaussian likelihood $N(0, \sigma_\omega^2\bI)$, and $p\big(f\big|\mu \big)$ is the \gls{CGP} likelihood specified in (\ref{eq:mono_gp}), i.e.:
\begin{align}
    p(f|\mu) = 
    \phi \Big(
    F, f \Big| 
    \begin{bmatrix} \Phi_\epsilon(.|\mu) \\ \phi_\epsilon(.|\mu) \end{bmatrix},
    \begin{bmatrix} 
            k & \partial_{\bz'} k \\
            \partial_{\bz} k & \partial_{\bz}\partial_{\bz'} k
    \end{bmatrix}
    \Big)
    *
    \Phi_\sigma(F)\Phi_\sigma(1-F)\Phi_\sigma(f),
\end{align}
where $\Phi_\epsilon$ and $\phi_\epsilon$ are the model \gls{CDF} and \gls{PDF} of the $\delta$-agumented ensemble (\ref{eq:model_system}).

\subsection{Hyperparameters}
\label{sec:hyper}

\gls{BNE}'s hyper-parameters are the Mat\'{e}rn length-scale parameters $l_\delta$ and $l_G$, and the prior variances $\sigma_\omega$ and $\sigma_\epsilon$. Consistent with the existing \gls{GP} approaches, we place the inverse-Gamma priors on the $l_\delta$ and $l_G$ and the Half Normal priors on $\sigma_\omega$ and $\sigma_\epsilon$ \citep{team_stan_nodate}, i.e.:
\begin{align*}
l_\delta &\sim invGamma(\alpha_\delta, \beta_\delta)
\quad
l_G  \sim invGamma(\alpha_G, \beta_G)
\end{align*}
where $\alpha$, $\beta$ where chosen so the prior probability for $l$ falling into a desired range $[l_{lower}, l_{upper}]$ is high. In this work, we set $l_{lower}=2$ and $l_{upper}=10$ such that $P_{invGamma}(l \in [2, 10]|\alpha, \beta)=0.98$ for both $l_\delta$ and $l_G$.  Finally, we use the weakly informative half-Gaussian priors for the variance parameters:
\begin{align*}
\sigma_\omega &\sim HalfNormal(0, 5)
\quad
\sigma_\epsilon \sim HalfNormal(0, 5)
\end{align*}

\subsection{Computation}

To fully capture the model uncertainty encoded in the posterior distribution, 
We perform posterior inference using \gls{HMC} \citep{neal_mcmc_2012}, and we use the adaptive step size proposed in \citep{andrieu_tutorial_2008} with implementation available in TensorFlow Probability \citep{dillon_tensorflow_2017}. Given data $\Dsc$ of size $N$, we first estimate the value of the hyper-parameters $\{l_\delta, l_G, \sigma_\omega, \sigma_\epsilon\}$ through an empirical Bayes approach by maximizing the posterior likelihood regularized by the hyper-parameter priors specified in \ref{sec:hyper}. We then perform full MCMC with respect to the posterior likelihood (\ref{eq:bne_posterior}), fixing the hyperparamters to their estimated values from the empirical Bayes procedure.

The computation complexity of sampling from \gls{BNE} posterior is $O(N^3)$ due to the need of inverting \gls{GP} kernel matrices. In the case of very large datasets, we consider the simple parallel MCMC scheme proposed in \cite{li_simple_2017} which is dedicated to estimating posterior quantiles (i.e. the inverse \gls{CDF}s). This method divides the dataset into $K$ subsets and run MCMC with respect to an adjusted posterior in parallel in each subset. As a result the computation complexity is reduced to $O(N^3/K^3)$ in the case of $K$ machines, or $O(N^3/K^2)$ in the case of a single machine.

==> sections/inference_old.tex <==
\section{Calibrated Inference}
\label{sec:inference}

\begin{comment}
For uncertainty quantification to be meaningful in practice, we'd like to perform inference in a way such that model's predictive uncertainty honestly reflects the empirical distribution of the data. To this end, we notice the following:
\begin{itemize}
\item As shown in the decomposition formula (\ref{eq:unc_decomp}), only the aleatoric component of a Bayesian model's predictive distribution is dedicated to describe data's empirical distribution. Consequently, a sound inference procedure should take care in matching \textit{only} the aleatoric component of the posterior predictive to the empirical distribution.
\item Traditional \gls{MLE} framework struggles in producing accurate uncertainty estimates. This is partially due to the fact that the \gls{MLE} methods use \gls{KL} divergence as the statistical distance between model and data $KL(F, \Fbb) = \int \big[ log \, d\Fbb(Y|\bx) - log f(y|\bx) \big] d\Fbb(y, \bx)$. In the presence of even slight irregularity in data distribution (e.g. outliers, heavy tail, etc), KL are known to tend to over-stretch its predictive distribution to capture all observations in the tail in order to avoid the infinite penalty in its $- log f(y|\bx)$ term \citep{ghosh_robust_2016, nakagawa_robust_2018}. Consequently in practice, \gls{MLE}-based methods are observed to tend to assign improperly large amount of probability mass to extreme events \citep{hoeting_bayesian_1999, thomas_bayesian_2007, bishop_bayesian_2008} and to over-disperse its  probability mass over the feature space \citep{ott_analyzing_2018}. Morever, even when the data are normally distributed, \gls{MLE} approaches are still known to produce biased variance estimates \citep{harville_maximum_1977}.
\end{itemize}
Above observations motivate the design of new inference framework that uses careful choice of statistical distance to achieve accurate quantification in the correct component (i.e. the aleatoric component) of model's predictive uncertainty. In particular, we consider the \gls{CvM} distance \citep{anderson_distribution_1962} which measures the $L_2$ distance between the model and the empirical \glspl{CDF}: 
\end{comment}
As it is well known in the generative model literature, for a model that specifies a flexible random component, the inference objective $l(y|x, \Theta) = D \Big[ F(y|\bx, \Theta), \;\Fbb(y|\bx) \Big]$ needs to be designed carefully for the inference procedure to reliably capture the data distribution \citep{arjovsky_towards_2017, arjovsky_wasserstein_2017}.
We introduce \textbf{Calibrated Inference}, a novel Bayesian learning  approach to achieve accurate and principled uncertainty quantification.
%estimation of aleatoric uncertainty (i.e. the model \gls{CDF} $F(y|\bx, \Theta)$) and principled quantification of epistemic uncertainty.
Specifically, it designs an inference objective $l(y|\bx, \Theta)$ that enforces the $L_2$ consistency between $F(y|\bx, \Theta)$ and the data distribution $\Fbb(y|\bx)$, and quantifies epistemic uncertainty by deriving the posterior distribution of $\Theta$ for solving the decision-theoretic problem of minimizing $l(y|\bx, \Theta)$.

\textbf{Accurate Aleatoric Uncertainty via CvM Distance}
%In principle, to produce accurate uncertainty quantification, model parameters  $\Theta$ should be estimated in a way that the model \gls{CDF}  $F(y|\bx, \Theta)$ is maximally consistent with the empirical distribution $\Fbb(y|\bx)$ with respect to a proper statistical distance $D$, i.e. minimizing
%\begin{align*}
%l(y|x, \Theta) = D \Big[ F(y|\bx, \Theta), \;\Fbb(y|\bx) \Big].
%\end{align*}
The classic choice for the inference objective $l(y|x, \Theta)$ is the \gls{KL} divergence $KL(y|\bx, \Theta) = \int \big[ log \, d\Fbb(y|\bx) - log f(y|\bx, \Theta) \big] d\Fbb(y, \bx)$, which gives rise to the classic \gls{MLE} framework. However, \gls{KL} are known to produce improper uncertainty quantification in the presence of even mild irregularity in data distribution (e.g. outliers, heavy-tailedness, etc). In these cases,  \gls{KL} tend to over-stretch its predictive distribution to capture all observations in the tail, in order to avoid the infinite penalty in its log term \citep{ghosh_robust_2016, nakagawa_robust_2018}. Consequently in practice, \gls{MLE}-based methods are observed to assign improperly large amount of probability mass to extreme events \citep{hoeting_bayesian_1999, thomas_bayesian_2007, bishop_bayesian_2008} and over-disperse the   probability mass in its model \gls{CDF} over the feature space \citep{ott_analyzing_2018}. 

In this work, we consider augmenting the original \gls{KL}-based $l(y|x, \Theta)$ with the \gls{CvM} distance \citep{anderson_distribution_1962}, i.e. the $L_2$ distance between the model and the empirical \glspl{CDF}. So our inference objective is:
\begin{align}
l(y | \bx, \Theta) &= KL(y | \bx, \Theta ) + \lambda * CvM(y | \bx,\Theta ), 
\label{eq:calibrated_divergence}
\end{align}
where 
\begin{align*}
CvM(y|\bx, \Theta) = \int \big[ F(y|\bx, \Theta) - \Fbb(y|\bx) \big]^2 d\Fbb(y, \bx), 
%\label{eq:cvm}
\end{align*}
and $\lambda > 0$ is a regularization parameter balancing the trade-off between $KL$ and $CvM$. We term $l(y | \bx, \Theta)$ the \textit{calibrated divergence}. It can be undersood as a regularized log likelihood with a penality term (i.e. \gls{CvM}) that measures model's quality in uncertainty quantification, or as a multi-task learning objective where model $F(y|\bx, \Theta)$ is tasked with both achieving good model fit with respect to \gls{KL}, and achieving accurate  uncertainty quantification with respect to \gls{CvM}.

Compared to \gls{KL}-only inference, incorporating \gls{CvM} into the inference objective $l(y|\bx, \Theta)$ improves the model's quality in uncertainty quantification. This is because minimizer of \gls{CvM} achieves accurate uncertainty quantification in its predictive intervals \citep{gneiting_strictly_2007}. Specifically, \gls{CvM} measures the distribution distance by comparing the predictive quantiles outputted by the model \gls{CDF} $F$ to those in the empirical distribution $\Fbb$ (recall that \gls{CDF} is the inverse quantile function). As a result, \gls{CvM} enforces model estimate to produce predictive intervals that are consistent with those in the empirical distribution. In comparison, \gls{KL} measures distribution distance by comparing $log dF$ to $log d \Fbb$, which does not directly compare predictive quantiles, and tend to  over-emphasis differences in the low probability regions of $F$ (since in these regions $|log dF|$ is large), which is not optimal for the purpose of uncertainty quantification. For this reason, \gls{CvM} is commonly preferred as a quality measure for assessing probablistic forecast's predictive uncertainty under the name \gls{CRPS} \citep{gneiting_strictly_2007}, and is estimated empirically as $\widehat{CvM}(y | \bx, \Theta) \approx
\frac{1}{M}\sum_{j=1}^M \big[ F(y_j|\bx, \Theta) - \Ibb(y < y_j|\bx) \big]^2$, where $y_j \in \Ysc$ are Monte Carlo sample points chosen by user. 
%Additionally, as we will show, under \gls{BNE}, performing inference with respect to \gls{CvM} simplifies the estimation for model's random component into a classic Gaussian process regression problem, which is a well-studied estimation problem with many high-quality inference algorithms available \citep{cheng_variational_2017, liu_when_2018}.

%Empirically, given $\{y_j\}_{j=1}^M$ the user-specified Monte Carlo sample points, the CvM distances is estimated as \citep{gneiting_strictly_2007} $\widehat{CvM}(y | \bx, \Theta) \approx
%\frac{1}{M}\sum_{j=1}^M \big[ F(y_j|\bx, \Theta) - \Ibb(y < y_j|\bx) \big]^2$. \gls{CvM} in this form is known as the \gls{CRPS} and is a standard measure in assessing a predictive distribution's quality in uncertainty quantification \citep{gneiting_probabilistic_2007}.


%\gls{CvM} is a natural choice for measuring a model's quality in uncertainty quantification. It compares the predictive quantiles outputted by the model $F$ to those in the empirical distribution. Consequently, since predictive interval is consistented of predictive quantiles, a model that minimizes \gls{CvM} will generate predictive credible intervals that are close to achieve their nominal coverage probability (e.g. we say a $90\%$ credible interval achieves nominal coverage when it indeed contains the true outcome $90\%$ of the time), which corresponds to the classical notion of accurate predictive uncertainty. 
%Furthermore, compared to \gls{KL}, the \gls{CvM} distance focuses on capturing the majority mass of the empirical distribution, and is known to be a more robust divergence in the robust statistics literature \citep{millar_robust_1981, selten_axiomatic_1998, basu_statistical_2011}.


Under \gls{BNE}, we can express the $l(y | \bx, \Theta)$ in  (\ref{eq:calibrated_divergence}) as:
{\footnotesize  
  \setlength{\abovedisplayskip}{6pt}
  \setlength{\belowdisplayskip}{\abovedisplayskip}
  \setlength{\abovedisplayshortskip}{0pt}
  \setlength{\belowdisplayshortskip}{3pt}
\begin{align*}
\hat{l}(y &| \bx, \Theta) = \\
& \bigg\{ - log \, f(y|\bx, \Theta) \bigg\} + 
\bigg\{ \frac{\lambda}{M} \sum_{j=1}^M 
\Big[ G \big[ F_S(y_j|\bx, \Phi) \big]  - \Ibb(y < y_j|\bx) \Big]^2
\bigg\}, \nonumber
\end{align*}
}%
where $f(y|\bx, \Theta)$ is the model CDF (See \ref{sec:calib_likelihood_deriv} for derivation). As shown, $\hat{l}$ is decomposed into two parts: the log likelihood that measures the prediction function's goodness of fit (the first bracket), and %a "penalized" 
the log likelihood of Gaussian process regression for $G$ (the second bracket) that measure's model's quality in uncertainty quantification
%, where the penalty term $g \big[ F_S(y|\bx, \Phi)\big]$ makes sure that $G$ is estimated in a way that it still contributes to maximizing the overall model log likelihood $f = g(F_S(y|\bx, \Phi)) * f_S(y|\bx, \Phi)$
.

%Specifically, this penalized likelihood matches the model CDF $F(y|\bx, \Theta) = G \circ F_S(y|\bx)$ to the empirical CDF $\Ibb(y < y_j|\bx)$ under the constraint that $g \big[ F_S(y|\bx)\big]$ (the likelihood term that is responsible for calibrating model \gls{PDF}) still contributes to maximizing the overall model likelihood $f = g \big[ F_S(y|\bx)\big] * f_S((y|\bx))$.
 
% In practice, a prudent strategy is to first "pre-train" the model under the traditional \gls{MLE} framework by fixing $\lambda=0$ and $G=I$ (the identity function), and then "fine-tune" model's uncertainty estimates by updating model posterior with respect to the full calibrated divergence.


%For the rest of this section, in Section \ref{sec:infer_framework}, we complete this new framework by introducing method to perform principled posterior inference with respect to the \gls{CvM}-augmented statistical distance, and explain how the proposed method achieves targeted calibration with respect to model's aleatoric uncertainty. Then, in Section \ref{sec:vi}, we propose \glsreset{CVI}\gls{CVI} which scales up this new inference method to real-world sized problems.

\textbf{Quantify Epistemic Uncertainty via Model Posterior}
%\subsection{Posterior Inference with Calibrated Divergence}
%\label{sec:infer_framework}
To quantify model's epistemic uncertainty in minimizing $l(y | \bx, \Theta)$ under finite data, we derive the posterior distribution for model parameters $\Theta$. For a given loss $l(y | \bx, \Theta)$, it can be shown that the posterior distribution for the $\Theta$ that minimizes $l(y | \bx, \Theta)$ is \cite{bissiri_general_2016}:
\begin{align}
f(\Theta | \{y, \bx\}) & \propto 
exp \Big(-l(y | \bx, \Theta) \Big) f(\Theta).
\label{eq:calibrated_posterior}
\end{align}
If setting $l(y | \bx, \Theta)$ to \gls{KL}, above posterior update rule corresponds exactly to that in the classic Bayesian inference. Authors of \cite{bissiri_general_2016} showed that the posterior in (\ref{eq:calibrated_posterior}) is not an approximation, neither is it a pseudo-posterior, but rather a valid representation of model's posterior  uncertainty in choosing the optimal parameters $\Theta=\{ G, \bdelta, \bmu, \bepsilon \big\}$ that minimize the global risk $l(y | \bx, \Theta)$ in finite data. Consequently, by following the above update rule, the interpretation of the posterior uncertainty in $\Theta$ coincides exactly with that of the epistemic uncertainty. 

%which minimizes the risk functional $L(f | y, \bx) = \int l(y | \bx, \Theta) f(\Theta)$ is
%Therefore the inference is \textit{optimal} in the decision-theoretic sense.

%Consequently, we see that by including \gls{CvM} into the inference objective, performing model update according to (\ref{eq:calibrated_posterior}) indeed results in a model posterior that  calibrates model's aleatoric uncertainty toward the empirical distribution. This is because the model posterior estimated through (\ref{eq:calibrated_posterior}) represents model's posterior belief in minizing the \gls{CvM} distance which matches model's distribution function $F(y|\bx, \Theta)$ to the empirical distribution $\Fbb$. Notice that $F(y|\bx, \Theta)$ indeed represents model's aleatoric uncertainty in its predictive distribution, since it quantifies the variation in the predicted $y$ when holding all the other model parameters $\Theta=\{S, \bmu, \bdelta, \sigma_\epsilon\}$ fixed.


\textbf{Calibrated Variational Inference} Finally, we enable scalable variational inference for the calibrated posterior in (\ref{eq:calibrated_posterior}) by deriving its \gls{ELBO}. For a variational family $q_{\bPsi}(\Theta)$ indexed by parameters $\psi$, we  derive \gls{ELBO} by treating $\hat{l}(y | \bx, \Theta)$ as the model's log likelihood, which gives:
\begin{align*}
\Lsc(f, & q_{\bPsi}|\{\bx, y\}) \\
= \; & 
\bigg\{
E \Big( -log \, f(y|\bx, \bTheta) \Big) + KL \Big( q_{\bPsi}(\bTheta), f(\bTheta) \Big) \bigg\} + 
 \nonumber \\
& 
\bigg\{
\frac{\lambda}{M}\sum_{j=1}^M E \Big( \big[ F(y_j|\bx, \bTheta) - \Ibb(y < y_j|\bx) \big]^2
\Big)
\bigg\},
\end{align*}
where all expectations are taken over $q_{\bPsi}(\bTheta)$ (see Appendix \ref{sec:calib_elbo_deriv} for derivation). We term the variational inference with respect to above \gls{ELBO} as the \gls{CVI}, since it can be understood as minimizing a regularized version of the the traditional \gls{ELBO} (first bracket) with a penalty term (second bracket) measuring the $q_{\Psi}$'s quality in uncertainty quantification using \gls{CvM}. Inference with respect to $\Lsc(f, q_{\bPsi}|\{\bx, y\})$ proceeds with stochastic gradient descent \citep{paisley_variational_2012}.

==> sections/related.tex <==
\section{Discussion and Related Work}
\label{sec:related}

\Gls{UQ} has a long history in robust engineering system design \citep{beyer_robust_2007} , financial investment management \citep{guiso_investment_1999}, and weather and climate forecast \citep{qian_uncertainty_2016}, where high-risk decisions and critical projections are made in the presence of noise and uncertainty. The exact goals of \gls{UQ}, while varying slightly by discipline, generally fall under one of the two categories: (i) \textbf{Accurate Uncertainty Estimation} to properly characterize a model's aleatoric and epistemic uncertainties for the purpose of reliable prediction, and (ii) \textbf{Uncertainty / Model Error Decomposition} to identify the sources of model error and uncertainty in the current system, for the purpose of uncertainty reduction and model improvement. We review existing work under these two categories in the following two subsections. Ensemble learning is becoming a standard modeling technique in many of these areas, with the type of base model predictors $\{f_k\}_{k=1}^K$ ranging from deterministic (e.g., rule-based expert systems \citep{creamer_automated_2010}) to probablistic (e.g. multi-model ensemble of perturbed physics simulations \citep{tebaldi_claudia_use_2007, garaud_uncertainty_2012, sanderson_uncertainty_2018}). Although our framework in (\ref{eq:model_orig}) assumes deterministic base models $f_k$, it can be readily adapted to probablistic predictors by assuming $\epsilon$ to be the weighted mixture of the probablistic component of the base models.

\subsection{Uncertainty Estimation}

The goal of uncertainty estimation is to properly characterize both  model's aleatoric and epistemic uncertainties. Specifically, in regions that are well represented by the training data, a model's aleatoric uncertainty should acurately capture the data's empirical distribution (i.e., calibration \citep{gneiting_strictly_2007}), while in regions unexplored by the training data, the model's epistemic uncertainty should elevate naturally to capture model's lack of confidence in prediction (i.e., out-of-distribution generalization \citep{lakshminarayanan_simple_2017})
%, while the aleatoric uncertainty should gracefully backs off to certain prior distribution
.

\textbf{Estimating Epistemic Uncertainty} Ensemble methods are often used as a technique to estimate the parametric uncertainty \citep{breiman_bagging_1996, lakshminarayanan_simple_2016} and to mitigate the structure uncertainty  \citep{breiman_stacked_1996, pinder_efficient_2009} of its base models. However, there exists less work in quantifying the epistemic uncertainty of an ensemble model itself. To this end, there are  frequentist approach in deriving a model's asymptotic distribution \citep{mentch_quantifying_2014}, Bayesian approaches that place structural prior on the model parameters \citep{chipman_bayesian_1998, kim_bayesian_2012, bishop_bayesian_2008, waterhouse_bayesian_1996, li_ensemble_2017, yao_using_2018}, and Monte Carlo methods that perturb model parameters randomly and propagate such parameter uncertainty forward in time through dynamic models  \citep{tebaldi_claudia_use_2007, garaud_uncertainty_2012, sanderson_uncertainty_2018}. Our work distinguishes from previous literature in that it uses Bayesian nonparametric methods to quantify the epistemic uncertainty in an ensemble model, with an special focus on quantifying the structural uncertainty. 

Compare to other approaches, Bayesian nonparametric methods (e.g. Gaussian process) are especially well suited for quantifying the epistemic uncertainty of a model, since its predictive variance is explicitly characterized by the distance from the training data  \citep{rasmussen_gaussian_2006}. Specifically, our approach in quantifying a model's structural uncertainty is inspired by two class of model calibration techniques: the \textit{computer model calibration}  \citep{kennedy_bayesian_2001} which calibrates a model's sysmatic component using an Gaussian process, and the \textit{probablistic calibration} \citep{niculescu-mizil_predicting_2005, kuleshov_accurate_2018, song_non-parametric_2018} which calibrates a  model's random component (e.g. the predictive CDF) using regression. Our method subsumes previous work by unifying these two empirically successful practices into one coherent Bayesian model, which enables end-to-end inference through a rigourous
%, decision-theoretic 
treatment of the modeling framework, and allows principled quantification of structural uncertainty by performing Bayesian inference 
% to minimize a generalized statistical divergence 
\citep{basu_statistical_2011}. Furthermore, we give explicit consideration to the model's out-of-distribution behavior in uncertainty quantification, which has been lacking in the calibration literature.

\textbf{Estimating Aleatoric Uncertainty}

There exists two common approaches in accurately estimating aleatoric uncertainty: model-based and inference-based. Model-based approaches capture aleatoric uncertainty by specifying a reasonable model for the random component. Common methods under this approach can be either `parametric' by assuming the data arise from a known distribution family (e.g. use heterogenous Gaussian for handling heterogeneity\citep{lakshminarayanan_simple_2016}, use Student's t for handling heavy-tailedness \citep{shaham_provable_2016} , use log-normal for asymmetry \citep{vandal_quantifying_2018}, etc), or `nonparametric' by deploying a flexible model without explicit assumption about data distribution (e.g. infinite Gaussian mixture \citep{rasmussen_infinite_2001} or implicit generative models \citep{mohamed_learning_2016}). Inference-based approaches, on the other hand, improve model's quality  in uncertainty quantification by modifying the inference objective with certain uncertainty metrics, which can be the coverage probability of predictive intervals \citep{pearce_high-quality_2018}, proper scoring rules \citep{lakshminarayanan_simple_2017, yao_using_2018, liu_adaptive_2018-1} or the kernelized calibration errors  \citep{kumar_trainable_2018}. Recognizing that the correct quantification of predictive uncertainty requires both a flexible model and also a carefully-designed inference procedure, our method combines these two approaches under a Bayesian framework. Specifically, 
%our inference method can be considered as a Bayesian generalization of \citep{kumar_trainable_2018} but using \gls{CRPS} as the calibration loss, while 
our modeling approach is distinct from the previous model-based methods in that our model is "semi-parametric" (i.e. the final model $F=G \circ \Phi$ is the nonparametric augmentation ($G$) of a parametric distribution family $\Phi$). Consequently, our model exhibits better convergence behavior than the other assumption-free methods (especially when $\Phi$ is specified approximately correctly), and is able to avoid model bias when the parametric assumption in $\Phi$ is violated. At the same time, our model is principled in that the model for $F=G \circ \Phi$ is designed to obey the mathamatical constrains (e.g. monotonicity, smoothness, etc) of distribution functions, and is easier to train when compared to the other nonparametric random-component models due to being an Gaussian process.

A work that is closely related to BNE is \cite{dasgupta_geometric_2017}, which also uses flexible transformations to augment a parametric model to better estimate the aleatoric noise. There are two main differences between BNE and the two-step approach in \citep{dasgupta_geometric_2017}: (1) the exact type of transformation used and (2) the inference method for the ensemble parameters $\omega$. 
%As a result, the two methods differ in the interpretability of the transformation parameter, and in the estimation quality for ensemble parameter $\omega$. 
Specifically, the transformation in BNE $G_{\bx}:\Phi(.|\bx) \rightarrow F^*(.|\bx)$ is an operator between distribution functions, while the transformation in  \cite{dasgupta_geometric_2017} is a diffeomorphism $\Gamma_{\bx}: y \rightarrow y'$ acting on the response space $y, y' \in \Ysc$. As a result, the PDFs for the two models are $f(y|\bx, \mu) 
= \deriv{y}\Phi\big(\bGamma_{\bx}(y)|\bx, \hat{\bomega}\big) 
= \phi\big(\bGamma_{\bx}(y)|\bx, \hat{\bomega} \big) 
* \bgamma_{\bx}(y)$ (Dasgupta et al), and $
f(y|\bx, \mu) 
= \deriv{y}\bG_{\bx}\big(\Phi(y|\bx, \bomega)\big) 
= \bg_{\bx}\big(\Phi(y|\bx, \bomega)\big)* \phi(y|\bx, \bomega)
$ (this work), where $g_\bx=\deriv{\Phi} G_\bx$ and $\gamma_\bx=\deriv{y}\Gamma_\bx$.
%{\footnotesize
%\begin{alignat*}{5}
%f(y|\bx, \mu) 
%&= \deriv{y}\Phi\big(\bGamma_{\bx}(y)|\bx, \hat{\theta}\big) 
%&& = \phi\big(\bGamma_{\bx}(y)|\bx, \hat{\bomega} \big) 
%&& * \bgamma_{\bx}(y),
%\qquad && \mbox{(Dasgupta et al)}
%\\
%f(y|\bx, \mu) 
%&= \deriv{y}\bG_{\bx}\big(\Phi(y|\bx, \theta)\big) 
%&& = \bg_{\bx}\big(\Phi(y|\bx, \bomega)\big) 
%&& * \phi(y|\bx, \bomega)
%\qquad && \mbox{(this work)}.
%\end{alignat*}}
As shown, the two models share a similarity in that their PDFs are the product of $\phi$ (a Gaussian PDF) and the derivative of a transformation function. However, their PDFs' exact expressions are in fact different. Comparing the two models, both models are  flexible in learning the data-generating $F^*$, while the construction in this work is better posed for uncertainty quantification in ensemble learning for two reasons: (1) Interpretability: $G_\bx$ is a transformation that directly "fixes" the original likelihood $\Phi$, which allow us to diagnose the misspecification in original likelihood by inspecting $G_{\bx}[\Phi]-\Phi$. This is not easy to do under the formulation of Dasgupta et al; (2) Estimation quality for the ensemble weights $\bomega$. Since \cite{dasgupta_geometric_2017} estimates $\bomega$ under the original parametric model, the resulting estimate $\hat{\bomega}$ can be biased if the original likelihood is misspecified. In comparison, our model estimates $\bomega$ under the flexible BNE likelihood to avoid biased inference.

\subsection{Identifying Sources of Model Error and Uncertainty}
The goal of uncertainty and error decomposition is to identify the sources of uncertainty and modeling misspecification in the current system, and to quantify their impact on the model output. The standard approach to uncertainty decomposition is to attribute the model's total predictive variance to the corresponding uncertainty sources using either analytical approaches (e.g. using either the analysis of variance (ANOVA) techniques \citep{yip_simple_2011, garaud_automatic_2011, bosshard_quantifying_2013} or the law of total variance as in \citep{depeweg_decomposition_2018} and in this work), or Monte Carlo simulation by reverse-propagating the predictive uncertainty backward from the model output to model parameters when the base predictors are differential equations (e.g. the \textit{reverse ensemble streamflow prediction} method in hydrological modeling \citep{wood_ensemble_2008}). 

Compared to uncertainty decomposition, error decomposition (i.e. identifying the sources of model misspecification and quantify their impact on prediction) is a more difficult task. In econometrics, this problem is being studied by an ongoing body of literature in the context of time-series modeling \citep{curdia_correlated_2010, del_negro_monetary_2009, inoue_identifying_2015, monti_can_2015, haan_agnostic_2018, paccagnini_dealing_2017}. The majority of these methods follow a \textit{parameter augmentation} approach, i.e. augmenting the possibly misspecified model components with additive / multiplicative random effects \citep{curdia_correlated_2010, del_negro_monetary_2009, inoue_identifying_2015} or with auxilary latent random variables \citep{monti_can_2015}, then detecting the existence of model misspecification by conducting hypothesis tests for the augmentation parameters \citep{monti_can_2015, haan_agnostic_2018}. The drawback of this approach is that the augmentation parameters still need to be specified correctly to capture the data's empirical distribution, therefore  misspecification may still exist after augmentation, which may render the conclusions drawn from the hypothesis tests invalid. Our method improves on these approaches by nonparametrically augmenting both the model's prediction and distribution function, thereby avoid making any explicit assumption about the augmentation parameters. Furthermore, since our model explicitly quantifies structural uncertainty, our method also provides a principled framework to comprehensively assess both the magnitude and the likelihood of different types of model misspecification, as well as their impact on different aspects of the predictive distribution. These features have been lacking in the previous literature.


\begin{comment}
\clearpage
 \textbf{Uncertainty Quantification} \citep{sullivan_introduction_2015, u.s._department_of_energy_scientific_2009, garaud_uncertainty_2012} 
 \begin{itemize}
\item Areas used, engineering system design, financial investment management \citep{guiso_investment_1999}, weather and climate forecast.
\item Primary goal: accurate quantification of aleatoric uncertainty for reliable prediction, and identify sources of model error and uncertainty for uncertainty reduction and model improvement.
\item Use of Ensemble Methods in these areas: probablistic: Multi-model Ensemble (MME) \citep{tebaldi_claudia_use_2007, sanderson_uncertainty_2018}, deterministic: rule-based expert systems \citep{creamer_automated_2010}.
\item Our framework assume deterministic base-models for generalizability. but can be adapted to probablistic ensemble by assuming $\epsilon$ to be the weighted mixture of the probablistic component of the base models.
\end{itemize}


\textbf{Uncertainty Estimation}
\begin{enumerate}
\item Metric: 
\begin{itemize}
\item Aleatoric: Calibration, proper scoring rule. \citep{gneiting_strictly_2007}.
\item Epistemic: Out-of-distribution generalization.
\end{itemize}
\item Method
\begin{enumerate}
\item Epistemic
\begin{itemize}
\item Ensemble itself is used to estimate parametric uncertainty \citep{breiman_bagging_1996, lakshminarayanan_simple_2016} and mitigate structural uncertainty \citep{breiman_stacked_1996, pinder_efficient_2009} in the base models.
\item Limited work in quantifying epistemic uncertainty in the ensemble learning itself (in constrast to neural network literature). 
In this work, we focus on epistemic uncertainty for ensemble learning through Bayesian nonparametric methods, with special focus on structural uncertainty.
\item There exists two types of general methods in structural uncertainty:
\begin{itemize}
\item Computer Model Calibration \citep{kennedy_bayesian_2001} (systematic component)
\item Probablistic Calibration \citep{kuleshov_accurate_2018, song_non-parametric_2018} (random component)
\end{itemize}
Our work subsume previous work by organizing them into one coherent model, and provided rigorous, decision-theoretic justification of this approach as a Bayesian inference for minimizing a general divergence.
\end{itemize}
\item Aleatoric
\begin{enumerate}
\item Model
\begin{itemize}
\item quantile regression (neural network \citep{tagasovska_frequentist_2018}, ensemble \citep{meinshausen_quantile_2006}). 
\item  flexible residual model with explicit parametrization e.g. mixture of Gaussians  \citep{bishop_pattern_2011}, or implicit generative model using neural nets \citep{depeweg_decomposition_2018}. 
\item Our approach distinguishes in that it is semi-parametric. Better convergence behavior if indeed Gaussian, but is able to overcome the parametric assumption when not. At the same time, obeys mathamatical constrains of distribution functions, thereby avoid overfitting. Finally much easier to train.
\end{itemize}
\end{enumerate}
\item Inference with alternative objective
\begin{itemize}
\item quality metrics for predictive intervals (Prediction Interval Coverage Probability (PICP) and Mean Prediction Interval Width (MPIW)) \citep{pearce_high-quality_2018} (problem)
\begin{itemize}
\item Problem: averaged individual conditional distributions across population (consequently, a lower bound on the actual calibration error), thus global calibration (e.g. globally shrinking width of predictive interval), although good performance when evaluated with global metric such as coverage probability, unclear if improvement over localized metric (e.g. CRPS) in the case of heterogenous noise, also unduly inference on out-of-distribution behavior. 
\end{itemize}
\item conditional entropy \citep{hafner_reliable_2018}.
\begin{itemize}
\item Problem: summarize conditional distributions either into scalar values, unable to distinguish between flexible model shape (unimodal and multimodal uncertainty profiles).
\end{itemize}
\item Calibration measure: proper scoring rule \citep{lakshminarayanan_simple_2016} or their kernelized version  \citep{kumar_trainable_2018}.
\end{itemize}
\item Other uncertainty: algorithmic uncertainty \citep{gupta_deep_2015, chen_statistical_2018}, data/input/distribution uncertainty \citep{malinin_predictive_2018} beyond the scope of this work.
\end{enumerate}
\end{enumerate}

\textbf{Identifying Sources of Model Error and Uncertainty}

\begin{enumerate}
\item detecting sources of uncertainty
\begin{enumerate}
\item Traditional: ANOVA (Gaussian likelihood over additive models) \citep{yip_simple_2011}\citep{garaud_automatic_2011}\citep{bosshard_quantifying_2013}
\item MCMC based approaches for PDE: reverse PPE \citep{wood_ensemble_2008},
\item Decomposition with Machine learning models: 
classic models: Neural network, heteroscedastic Gaussian noise \citep{kendall_what_2017}. GP \citep{mcallister_bayesian_2017}, 
More general approach with implicit models \citep{depeweg_decomposition_2018}.
\end{enumerate}
Quantification restricted to second moment. Due to not accounting for structural misspecification and uncertainty.
\item Detecting sources of misspecification: Econometrics \citep{inoue_identifying_2015, haan_agnostic_2018, paccagnini_dealing_2017}. cannot formally assess likelihood of misspecification. due to not discussing uncertainty.
\item Ours quantified structural error and associated uncertainty. Therefore can trace source, quantify impact on whole range of properties, and provide principled assessment for the likelihood of misspecification.
\end{enumerate}

\newpage

\textbf{Uncertainty quantification (UQ)} has a long history in engineering system design {\color{red} cite}, environmental modeling {\color{red} cite}, and numeric weather / climate forecasts  {\color{red} cite}, with the primary goals being (1) identifying different sources of modeling error and uncertainty in the current system, and (2) assessing their impact on model output 
\citep{u.s._department_of_energy_scientific_2009}. UQ is traditionally accomplished by \textit{forward uncertainty propagation}, i.e. by randomly perturbing components (e.g. initial conditions, model parameters) of a deterministic model in order to propogate stochasticity forward into model prediction {\color{red} cite}.



\begin{itemize}
\item Uncertainty quantification
\begin{itemize}
\item Long tradition in engineering systems for solving inverse problems and probablistic forcast for environment and climate modeling, central goal (1) identify sources of uncertainty (2) quantify impact on model output.
\item quantification method in ensemble learning
\begin{itemize}
\item forward uncertainty propagation, using Monte Carlo methods
\item Inverse uncertainty quantification
\end{itemize}
\end{itemize}
\item Accurate uncertainty estimation
\begin{enumerate}
\item metric: proper scoring rule. \citep{gneiting_strictly_2007} 
\item method:
\begin{enumerate}
\item in statistics, studied under the notion of robust statistics. To this end, the modeling philosophy: embed parametric model in more flexible model space through Bayesian nonparametric building blocks  \citep{watson_approximate_2016, robert_nonparametric_2016}, inference philosphy: robust estimation general distance \cite{parr_minimum_1980, basu_robust_1998} Bayesian extension \cite{ghosh_robust_2016, bissiri_general_2016}
\item in machine learning, model calibration, \citep{kennedy_bayesian_2001}
\citep{kuleshov_accurate_2018}
\citep{song_non-parametric_2018} 
\end{enumerate}
\item We subsume previous work:
\begin{enumerate}
\item model: 
\begin{enumerate}
\item unifying empirically succesful calibration techniques into one coherent Bayesian model, 
\item investigates their role in uncertainty decomposition and quantification, and developed methods and tools to (impact assessment).
\end{enumerate}
\item inference: 
\begin{enumerate}
\item rigourous theoretical justification through Bayesian inference for  general divergence minimization.
\item Developed principled posterior update algorithm for end-to-end inference that jointly achives model estimation and nonparametric calibration.
\item furthermore, practical use through variantional inference quantifying uncertainty (statistical distance + variational family).
\end{enumerate}
\end{enumerate}
\end{enumerate}

\end{itemize}
\end{comment}
